Position: Beyond Sensitive Attributes, ML Fairness Should Quantify Structural Injustice via Social Determinants

Algorithmic fairness research has largely framed unfairness as discrimination along sensitive attributes. However, this approach limits visibility into unfairness as structural injustice instantiated through social determinants, which are contextual variables that shape attributes and outcomes without pertaining to specific individuals. This position paper argues that the field should quantify structural injustice via social determinants, beyond sensitive attributes. Drawing on cross-disciplinary insights, we argue that prevailing technical paradigms fail to adequately capture unfairness as structural injustice, because contexts are potentially treated as noise to be normalized rather than signal to be audited. We further demonstrate the practical urgency of this shift through a theoretical model of college admissions, a demographic study using U.S. census data, and a high-stakes domain application regarding breast cancer screening within an integrated U.S. healthcare system. Our results indicate that mitigation strategies centered solely on sensitive attributes can introduce new forms of structural injustice. We contend that auditing structural injustice through social determinants must precede mitigation, and call for new technical developments that move beyond sensitive-attribute-centered notions of fairness as non-discrimination.

==> file/main/call_to_action.tex <==
In summary, the effects of social determinants cannot be replaced by centering mitigation strategies on sensitive attributes alone.
Reducing discrimination and/or disadvantage to pathways originating from sensitive attributes may induce a kind of thought inertia: it reinforces a habitual framing that is natural and intuitive, yet risks obscuring other critical drivers and technical approaches, e.g., the role of social determinants when capturing disadvantage, and the need for current causal fairness frameworks to meaningfully accommodate community- and context-level causal factors rather than treating social determinants as ordinary individual-level auxiliary attributes.

\subsection{Remark: Social Determinants and Sensitive Attributes Are Non-Interchangeable}
Reflecting on cross-disciplinary perspectives on social determinants (Section~\ref{main:cross_disciplinary_engagement}) alongside the technical choices used to frame metrics/inquiries in algorithmic fairness (Section~\ref{main:limit_technical_paradigm}), we identify a critical gap in the literature: the addressing of structural injustice is often operationalized in an incomplete or reductive manner, both conceptually and technically.

First, metrics that solely focus on sensitive attributes fail to capture the shifting and context-dependent influences of social determinants, in static and dynamic settings alike (Section~\ref{main:limit_technical_paradigm:stable_shifting}).
Second, framing discrimination primarily through edges/pathways originating from sensitive attributes can narrow the space of actionable interventions, implicitly encouraging ``interventions'' on individual identity rather than mitigation strategies that target structural and environmental drivers (Section~\ref{main:limit_technical_paradigm:obscure_mitigation}).
Third, despite their substantive importance, attributes related to social determinants are frequently excluded in practice (Section~\ref{main:limit_technical_paradigm:data_issue}).

Collectively, we argue for the need for fairness analyses to explicitly model and adapt to contextual variation, rather than treating social determinants as interchangeable with, or reducible to, sensitive attributes.
In following sections, we substantiate the practical urgency of this shift via three analyses: a theoretical model of college admissions, a U.S. Census demographic study, and a high-stakes domain application regarding breast cancer screening within an integrated U.S. healthcare system.
